HybEA: Hybrid Models for Entity Alignment

Entity Alignment (EA) aims to detect descriptions of the same real-world entities among different Knowledge Graphs (KG). Several embedding methods have been proposed to rank potentially matching entities of two KGs according to their similarity in the embedding space. However, existing EA embedding methods are challenged by the diverse levels of structural (i.e., neighborhood entities) and semantic (e.g., entity names and literal property values) heterogeneity exhibited by real-world KGs, especially when they are spanning several domains (DBpedia, Wikidata). Existing methods either focus on one of the two heterogeneity kinds depending on the context (mono- vs multi-lingual). To address this limitation, we propose a flexible framework called HybEA, that is a hybrid of two models, a novel attention-based factual model, co-trained with a state-of-the-art structural model. Our experimental results demonstrate that HybEA outperforms the state-of-the-art EA systems, achieving a 16% average relative improvement of Hits@1, ranging from 3.6% up to 40% in 5 monolingual datasets, with some datasets that can now be considered as solved. We also show that HybEA outperforms state-of-the-art methods in 3 multi-lingual datasets, as well as on 2 datasets that drop the unrealistic, yet widely adopted, one-to-one assumption. Overall, HybEA outperforms all (11) baseline methods in all (3) measures and in all (10) datasets evaluated, with a statistically significant difference.

==> tables/tab_ablation.tex <==
\begin{table*}[t]
\centering
\caption{Comparison of HybEA performance depending on embedding size and type of embedding used (SentenceBERT, LaBSE and random initialization). \textbf{Maybe need of gigaflops and time per epoch here ? Which dataset ?}}
\label{tab:embedding_ablation}
\begin{tabular}{|l|l|lll|lll|}
\hline
\multirow{2}{*}{}                              & \multirow{2}{*}{Embeddings size} & \multicolumn{3}{l|}{HybEA (basic)}                               & \multicolumn{3}{l|}{HybEA}                                     \\ \cline{3-8} 
                                               &                                  & \multicolumn{1}{l|}{H@1}   & \multicolumn{1}{l|}{H@10}  & MRR  & \multicolumn{1}{l|}{H@1}   & \multicolumn{1}{l|}{H@10}  & MRR  \\ \hline
\multirow{2}{*}{HybEA + SentenceBERT}          & 768                              & \multicolumn{1}{l|}{0.877} & \multicolumn{1}{l|}{0.962} & 0.90 & \multicolumn{1}{l|}{0.920} & \multicolumn{1}{l|}{0.969} & 0.93 \\ \cline{2-8} 
                                               & 300                              & \multicolumn{1}{l|}{0.871} & \multicolumn{1}{l|}{0.963} & 0.90 & \multicolumn{1}{l|}{0.913} & \multicolumn{1}{l|}{0.969} & 0.93 \\ \hline
HybEA + LaBSE                                  & 768                              & \multicolumn{1}{l|}{0.860} & \multicolumn{1}{l|}{0.953} & 0.89 & \multicolumn{1}{l|}{0.910} & \multicolumn{1}{l|}{0.969} & 0.93 \\ \hline
\multirow{2}{*}{HybEA + random initialization} & 256                              & \multicolumn{1}{l|}{0.854} & \multicolumn{1}{l|}{0.942} & 0.88 & \multicolumn{1}{l|}{0.901} & \multicolumn{1}{l|}{0.960} & 0.92 \\ \cline{2-8} 
                                               & 768                              & \multicolumn{1}{l|}{0.853} & \multicolumn{1}{l|}{0.933} & 0.88 & \multicolumn{1}{l|}{0.901} & \multicolumn{1}{l|}{0.952} & 0.92 \\ \hline
\end{tabular}
\end{table*}

==> tables/tab_complexity.tex <==

\begin{table*}[t]
\footnotesize
\centering
\caption{Performance of \syst\ variants per embedding size and type  (* indicates results only of the structural component).}
\vspace{-5pt}
\label{tab:embedding_complexity}



\begin{tabular}{|cl|c|c|cc|c|c|ccc|}
\hline
\multicolumn{2}{|c|}{}                                 &                                                                             &                                                                                & \multicolumn{2}{c|}{\textbf{Number of epochs (NoE)}}                                                                                                               &                          &                                                                                    & \multicolumn{3}{c|}{\textbf{\DOne}}                                                                                                           \\ \cline{5-6} \cline{9-11} 
\multicolumn{2}{|l|}{\multirow{-2}{*}{\textbf{Model}}}          & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Embedding} \\ \textbf{size}\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Time per} \\ \textbf{epoch (TpE)} \end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Factual} \\ \textbf{component}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}\textbf{Structural} \\ \textbf{component}\end{tabular} & \multirow{-2}{*}{\textbf{GFLOPs}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Overall Cost} \\ \textbf{(GFLOPs} $\times$ \textbf{TpE} $\times$ \textbf{NoE )}\end{tabular}} & \multicolumn{1}{c|}{\textbf{H@1}}                          & \multicolumn{1}{c|}{\textbf{H@10}}                         & \textbf{MRR}                         \\ \hline
\multicolumn{2}{|l|}{\textbf{\systK \  (w/o struct.)}}              & 768                                                                         & 157                                                                            & \multicolumn{1}{c|}{85}                                                           & 0                                                               & 95                       & 1268                                                                               & \multicolumn{1}{c|}{0.558}                        & \multicolumn{1}{c|}{0.612}                        & 0.79                        \\ \hline
\multicolumn{2}{|l|}{\textbf{\systK \  (w/o fact.)}}                & 768                                                                         & 32*                                                                             & \multicolumn{1}{c|}{0}                                                            & 85                                                              & 523*                      & 1423*                                                                               & \multicolumn{1}{c|}{0.753}                        & \multicolumn{1}{c|}{0.936}                        & 0.82                        \\ \hline
\multicolumn{2}{|l|}{\textbf{\systK \ }}                            & 768                                                                         & 32*                                                                            & \multicolumn{1}{c|}{230}                                                          & 325                                                             & 523*                      & 5439*                                                                               & \multicolumn{1}{c|}{\textbf{0.920}}               & \multicolumn{1}{c|}{\textbf{0.969}}               & \textbf{0.93}               \\ \hline
\multicolumn{2}{|l|}{\textbf{\systK \  Reduced}}    & 256                                                                         & 12*                                                                            & \multicolumn{1}{c|}{295}                                   & 175                                      & 129*                      &                                        271*                                            & \multicolumn{1}{c|}{0.913} & \multicolumn{1}{c|}{0.965} & 0.93 \\ \hline
\multicolumn{2}{|l|}{\textbf{\systK \  Light Full}} & 768                                                                         & 32*                                                                            & \multicolumn{1}{c|}{225}                                                          & 170                                                             & 523*                      & 2845*                                                                               & \multicolumn{1}{c|}{0.901}                        & \multicolumn{1}{c|}{0.953}                        & 0.92                        \\ \hline
\multicolumn{2}{|l|}{\textbf{\systK \  Light}}                      & 256                                                                         & 12*                                                                            & \multicolumn{1}{c|}{235}                                                          & 245                                                             & 129*                      & \textbf{379}*                                                                       & \multicolumn{1}{c|}{0.902}                        & \multicolumn{1}{c|}{0.961}                        & 0.92                        \\ \hline
\end{tabular}
\vspace{-5pt}
\end{table*}

% \usepackage{multirow}
%\begin{table*}[t]
%\centering
%\caption{\textcolor{red}{Comparison of systems' performance based on embedding size and type (Sentence-BERT, LaBSE and random).}}
%\label{tab:embedding_complexity}
%\begin{tabular}{|ll|l|l|l|lll|lll|}
%\hline
%\multicolumn{2}{|l|}{\multirow{2}{*}{\textbf{Model}}}        & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{Node embedding} \\ \textbf{size}\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{Time per} \\ \textbf{epoch (s)}\end{tabular}} & \multirow{2}{*}{\textbf{GFlops}} & \multicolumn{3}{c|}{\textbf{\DFive}}    & \multicolumn{3}{c|}{\textbf{\DOne}}   \\ \cline{6-11} 
%\multicolumn{2}{|l|}{}     &    & &       & \multicolumn{1}{l|}{\textbf{H@1}}   & \multicolumn{1}{l|}{\textbf{H@10}}  & \textbf{MRR}   & \multicolumn{1}{l|}{\textbf{H@1}}   & \multicolumn{1}{l|}{\textbf{H@10}}  & \textbf{MRR}   \\ \hline
%\multicolumn{2}{|l|}{\syst\ (w/o struct.)}    & 768  & & 95    & \multicolumn{1}{l|}{0.748} & \multicolumn{1}{l|}{0.769} & 0.91  & \multicolumn{1}{l|}{0.558} & \multicolumn{1}{l|}{0.612} & 0.79  \\ \hline
%\multicolumn{2}{|l|}{\syst\ (w/o fact.)}      & 768  & & 523   & \multicolumn{1}{l|}{0.974} & \multicolumn{1}{l|}{0.995} & 0.98  & \multicolumn{1}{l|}{0.753} & \multicolumn{1}{l|}{0.936} & 0.82  \\ \hline
%\multicolumn{1}{|l|}{\multirow{6}{*}{\syst}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Sentence-BERT embeddings \\on structural component\end{tabular}} & 768  & & 523   & \multicolumn{1}{l|}{0.996} & \multicolumn{1}{l|}{0.997} & 0.99  & \multicolumn{1}{l|}{0.920} & \multicolumn{1}{l|}{0.969} & 0.93  \\ \cline{3-11} 
%\multicolumn{1}{|l|}{}     &      & 300  & & 155   & \multicolumn{1}{l|}{-}     & \multicolumn{1}{l|}{-}     & -     & \multicolumn{1}{l|}{0.913} & \multicolumn{1}{l|}{0.969} & 0.93  \\ \cline{2-11} 
%\multicolumn{1}{|l|}{}     & \begin{tabular}[c]{@{}l@{}}LaBSE embeddings\\ on structural component\end{tabular}    & 768  & & 523   & \multicolumn{1}{l|}{-}     & \multicolumn{1}{l|}{-}     & -     & \multicolumn{1}{l|}{0.910} & \multicolumn{1}{l|}{0.963} & 0.93  \\ \cline{2-11} 
%\multicolumn{1}{|l|}{}     & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Random initialization\\ on structural component\end{tabular}} & 256  & & 129  & \multicolumn{1}{l|}{-}     & \multicolumn{1}{l|}{-}     & -     & \multicolumn{1}{l|}{0.902} & \multicolumn{1}{l|}{0.961} & 0.92  \\ \cline{3-11} 
%\multicolumn{1}{|l|}{}     &      & 768  & & 523   & \multicolumn{1}{l|}{-}     & \multicolumn{1}{l|}{-}     & -     & \multicolumn{1}{l|}{0.901} & \multicolumn{1}{l|}{0.953} & 0.92  \\ \hline
%\multicolumn{2}{|l|}{SelfKG}      & 768  & & 1     & \multicolumn{1}{l|}{0.961} & \multicolumn{1}{l|}{0.976} & 0.972 & \multicolumn{1}{l|}{0.542} & \multicolumn{1}{l|}{0.707} & 0.592 \\ \hline
%\multicolumn{2}{|l|}{ZeroEA}      & 512  & & 45    & \multicolumn{1}{l|}{0.969} & \multicolumn{1}{l|}{0.976} & 0.807 & \multicolumn{1}{l|}{0.466} & \multicolumn{1}{l|}{0.504} & 0.437 \\ \hline
%\end{tabular}
%\end{table*}

==> tables/tab_efficiency.tex <==
\begin{table*}[ht]
\centering
\caption{Efficiency of embedding-based EA methods: training + testing time (in seconds).}
\label{tab:efficiency}
\begin{tabular}{lrrrr} 
\hline
\textbf{Dataset} & \textbf{RREA(basic)} & \textbf{Knowformer} & \textbf{SelfKG} \\ 
\hline
\DOne        & 355.56 + 31.75 & 3,298.60 + 10.38 &  10,936.89 + 457.39\\ 
\DTwo        & 459.19 + 32.51 & 3,593.11 + 10.34 &  10,970.19 + 454.70\\ 
\DThree       & 360.52 + 31.01 & 2,567.17 + 10.30  &    11,087.39 + 586.50\\ 
\DFour        & 432.73 + 15.67 & 3,360.07 + 10.59   &   10,972.44 + 454.85 \\ 
\DFive        & 203.55 + 15.42 &  1,004.92 + 4.37 & 6,909.17 + 184.98\\ 
ICEWS-WIKI    & 1,567.48 +18.42 & 29,114.8 +6.01 & 10,175.62 + 226.21 \\
ICEWS-YAGO    & 1,731.06 + 65.93 & 46,843.75 +21.87 & 17,291.17+ 784.18 \\
\hline
\end{tabular}
\end{table*}





==> tables/tab_efficiency_per_component.tex <==
\begin{table*}[ht]
\centering
\caption{Meaning time per epoch of the different componant of HybEA}
\label{tab:efficiency}
\begin{tabular}{lrrrr} 
\hline
\textbf{Dataset} & \textbf{RREA(basic)} & \textbf{Knowformer} & \textbf{HybEA (w/o struct.)} \\ 
\hline
\DOne        & 0.22  & 32.81 & 65.44 \\ 
\DTwo        & 0.30 & 62.70 &  59.74 \\ 
\DThree       & 0.21 & 31.88 &  57.54 \\ 
\DFour        & 0.28 & 57.77 &  53.55 \\ 
\DFive        & 0.13  &  23.17 & 51.27 \\ 
\hline
\end{tabular}
\end{table*}





==> tables/tab_flops.tex <==
% \begin{table*}[t]
%     \centering
%     \caption{Evaluation of model efficiency in Giga FLOPS (GF) and time per epoch (in seconds), on the \DOne\ dataset.}
%     \label{tab:flops}
%     \begin{tabular}{c|cc}
%         \textbf{Model} & \textbf{\syst\ (w/o struct.)} & \textbf{\syst\ (w/o fact.)} \\ %& \textbf{Knowformer} \\ % & \textbf{BERT-INT} \\ 
%         \hline
%         \textbf{GF} & $95.90$ & $523.6$  \\ \hline %$129.17$ \\ \hline %& $0.121 \times 10^{-3}$ 
%         \textbf{Time per epoch (s)} & $404$ & $153$ \\  %$83$ \\ \hline %$447$ &
%     \end{tabular}
% \end{table*}



\begin{table}[t]
    \centering
    \caption{Evaluation of model efficiency in Giga FLOPS (GF) and time per epoch (in seconds), on the \DOne\ dataset. Maybe here we need HybEA, HybEA Light etc ??? \textbf{Guillaume:} Remove this table and report in table 6 ?}
    \label{tab:flops}
    \begin{tabular}{l|c|c}
        \textbf{Model} & \textbf{GF} & \textbf{Time per epoch (s)} \\ \hline
        \textbf{\syst\ (w/o struct.)}   & 95.90 & 404\\ \hline
        \textbf{\syst\ (w/o fact.)}     & 523.6 & 153 \\ 
    \end{tabular}
\end{table}
